Pauli component erasing quantum channels

Decoherence of quantum systems is described by quantum channels. However, a complete understanding of such channels, especially in the multi-particle setting, is still an ongoing difficult task. We propose the family of quantum maps that preserve or completely erase the components of a multi-qubit system in the basis of Pauli strings, which we call Pauli component erasing maps. For the corresponding channels, it is shown that the preserved components can be interpreted as a finite vector subspace, from which we derive several properties and complete the characterization. Moreover, we show that the obtained family of channels forms a semigroup and derive its generators. We use this simple structure to determine physical implementations and connect the obtained family of channels with Markovian processes.

==> decoh_set.tex <==
\section{The set of decoherence channels} % {{{
\todo{Aun no comenzar a escribir hasta que sepamos qeu queremos decir (si es
que queremos decir algo}
\begin{itemize}
\item Aca creo qe pueden ser puntos extremos de ese conjunto de canales
\item El conjunto dentro del conjunto de todos los canales (puntos extremos)
\end{itemize}
% }}}


==> prueba.tex <==
\section{Proof of a non-obvious consequence}
\label{app:proof}
Here we show that (\ref{eq:13}) implies (\ref{eq:14}). Since (\ref{eq:13}) holds for 
all $\vec\beta\in\Phi(\vec\alpha)$, we may choose a specific such $\vec\beta$, namely
$\beta_l=0$ for all $l\neq k$ and $\beta_k=\beta$, where $\beta$ is an arbitrary number
such that
\begin{equation}
\sa_{\alpha_k\beta}=1.
\end{equation}
This $\vec\beta$, as is readily verified, belongs to $\Phi(\vec\alpha)$, so that (\ref{eq:13})
indeed holds for this $\vec\beta$. On the other hand, it is then readily verified that, for this
$\vec\beta$, (\ref{eq:13}) reduces to (\ref{eq:14}), whcih therefore follows. 


































==> qudits.tex <==
\section{Higher dimensional systems} % {{{
\todo{Alejo o Jose Alfredo escriben aca. Se ponen de acuerdo y dejan a un responsable}
\begin{itemize}
\item Discuss what happens with general $d$ level systems and why it does not work
\item Linealidad de los eigenvalores de la matriz de Choi en función de las
$\tau_{j_1\ldots,j_n}$ de canales `\textit{component erasing}' de qudits. 
\item Discuss what happens with general $(2^k)^{\otimes n}$ level systems and
why it does work
\end{itemize}

\textcolor{jacolor}{
\begin{enumerate}
	\item Explicar cómo nuestro trabajo se generaliza trivialmente 
	para los sistemas de $d=(2^k)^{\otimes n}$ niveles.
	\item Describir el problema de $d=3$ con las matrices de Gell-Mann. El 
	problema es la no linealidad de los eigenvalores de la matriz de Choi en 
	función de las $\taus$.
	\begin{itemize}
		\item A diferencia de los PCE de qubits, la matriz de Choi de GMCE de qutrits
		no se diagonaliza con las matrices de GellMan.  
		\item El bloque problemático es el asociado a las matrices de GellMann diagonales.
		\item Mencionar sobre los operadores de Weyl.
	\end{itemize}
\end{enumerate}
}

% }}}

